Geometric Unsupervised Domain Adaptation for Semantic Segmentation

Simulators can efficiently generate large amounts of labeled synthetic data with perfect supervision for hard-to-label tasks like semantic segmentation. However, they introduce a domain gap that severely hurts real-world performance. We propose to use self-supervised monocular depth estimation as a proxy task to bridge this gap and improve sim-to-real unsupervised domain adaptation (UDA). Our Geometric Unsupervised Domain Adaptation method (GUDA) learns a domain-invariant representation via a multi-task objective combining synthetic semantic supervision with real-world geometric constraints on videos. GUDA establishes a new state of the art in UDA for semantic segmentation on three benchmarks, outperforming methods that use domain adversarial learning, self-training, or other self-supervised proxy tasks. Furthermore, we show that our method scales well with the quality and quantity of synthetic data while also improving depth prediction.

==> figures/camera.tex <==

% \begin{figure}[t!]
% \centering
% \subfloat[Real to virtual resizing]{
% \includegraphics[width=0.16\textwidth,height=2.0cm]{
% images/camera/pd_orig_rgb.png}
% \includegraphics[width=0.16\textwidth,height=2.0cm]{
% images/camera/pd_orig_depth.png}
% \includegraphics[width=0.16\textwidth,height=2.0cm]{
% images/camera/kitti_conv.png}
% } \\
% \vspace{-2mm}
% \subfloat[Virtual to real resizing]{
% \includegraphics[width=0.16\textwidth,height=1.2cm]{
% images/camera/pd_resize_rgb.png}
% \includegraphics[width=0.16\textwidth,height=1.2cm]{
% images/camera/pd_resize_depth.png}
% \includegraphics[width=0.16\textwidth,height=1.2cm]{
% images/camera/kitti_orig.png}
% } \\
% \vspace{-2mm}
% \subfloat[Virtual to real reprojection]{
% \includegraphics[width=0.16\textwidth,height=1.2cm]{
% images/camera/pd_conv_rgb.png}
% \includegraphics[width=0.16\textwidth,height=1.2cm]{
% images/camera/pd_conv_depth.png}
% \includegraphics[width=0.16\textwidth,height=1.2cm]{
% images/camera/kitti_orig.png}
% }
% \caption{Camera normalization trick. Virtual images (\textit{PD}) are $1936 \times 1216$ and real images (\textit{KITTI}) are $352 \times 1216$.}
% \label{fig:camera}
% \end{figure}



\begin{figure}[t!]
\centering
\subfloat[Real to virtual resizing]{
\includegraphics[width=0.16\textwidth,height=2.0cm]{
images/camera/pd_orig_rgb.png}
\includegraphics[width=0.16\textwidth,height=2.0cm]{
images/camera/pd_orig_depth.png}
\includegraphics[width=0.16\textwidth,height=2.0cm]{
images/camera/kitti_conv.png}
} \\
\vspace{-2mm}
\subfloat[Virtual to real resizing]{
\includegraphics[width=0.16\textwidth,height=1.2cm]{
images/camera/pd_resize_rgb.png}
\includegraphics[width=0.16\textwidth,height=1.2cm]{
images/camera/pd_resize_depth.png}
\includegraphics[width=0.16\textwidth,height=1.2cm]{
images/camera/kitti_orig.png}
} \\
\vspace{-2mm}
\subfloat[Virtual to real reprojection]{
\includegraphics[width=0.16\textwidth,height=1.2cm]{
images/camera/pd_conv_rgb.png}
\includegraphics[width=0.16\textwidth,height=1.2cm]{
images/camera/pd_conv_depth.png}
\includegraphics[width=0.16\textwidth,height=1.2cm]{
images/camera/kitti_orig.png}
}
\caption{Camera normalization trick. Virtual images (\textit{PD}) are $1936 \times 1216$ and real images (\textit{KITTI}) are $352 \times 1216$.}
\label{fig:camera}
\end{figure}

==> figures/diagram.tex <==

\begin{figure*}[t!]
\vspace{-4mm}
\centering
\subfloat[Real sample processing]{
\raisebox{9mm}{\includegraphics[width=0.45\textwidth,trim=110 140 90 120,clip]{images/diagram_real_hr.pdf}}
}
\subfloat[Virtual sample processing]{
\includegraphics[width=0.55\textwidth,trim=50 90 50 120,clip]{images/diagram_virtual_hr.pdf}
}
% \vspace{-2mm}
\caption{\textbf{Diagram of our proposed GUDA architecture} for geometric unsupervised domain adaptation using mixed-batch training of real and virtual samples. Each sample is processed independently (Secs. \ref{sec:real_sample} and \ref{sec:virtual_sample}), based on its level of available supervision, and the final losses are combined for the optimization step. }
\label{fig:diagram}
\vspace{-4mm}
\end{figure*}

==> figures/kitti.tex <==

\begin{figure*}[t!]
\centering
%\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-0-rgb_7_579612eb.png}}
%\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-0-inv_depth_7_43ecc726.png}}
%\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-0-inv_depths_43_dd51608a.png}}
%\\ \vspace{-3mm}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-176-rgb_7_06c3d3a5.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-176-inv_depth_7_ddf90ae0.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-176-inv_depths_43_1c3c0297.png}}
\\ \vspace{-3mm}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-528-rgb_7_d27982c2.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-528-inv_depth_7_53d61eb9.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-528-inv_depths_43_65cbe37e.png}}
\\ \vspace{-3mm}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-704-rgb_7_d90ea206.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-704-inv_depth_7_03dd3512.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-704-inv_depths_43_0ff36732.png}}
\\ \vspace{-3mm}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-880-rgb_7_79d440f9.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-880-inv_depth_7_012258a4.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_val_files-velodyne-880-inv_depths_43_dd0fb56f.png}}
\\ \vspace{-3mm}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-136-rgb_7_5a4cc9ba.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-136-inv_depth_7_fb0aaa08.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-136-inv_depths_43_b26273cb.png}}
\\ \vspace{-3mm}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-272-rgb_0_ab568b48.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-272-inv_depth_7_6e61d8b9.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-272-inv_depths_43_ce8b9cfe.png}}
\\ \vspace{-3mm}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-680-rgb_7_3047baeb.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-680-inv_depth_7_33cefcc5.png}}
\subfloat{\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-680-inv_depths_43_e1ae2569.png}}
\\ \vspace{-3mm}
\setcounter{subfigure}{0}
\subfloat[RGB]{
\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-544-rgb_7_73ad00ee.png}}
\subfloat[Monodepth2]{
\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-544-inv_depth_7_1c49c522.png}}
\subfloat[Ours]{
\includegraphics[width=0.32\textwidth,height=1.8cm]{images/kitti/media_images_val-KITTI_raw-eigen_test_files-velodyne-544-inv_depths_43_10876f6e.png}}
%\\ \vspace{-3mm}
%\subfloat[RGB]{
%\includegraphics[width=0.23\textwidth]{example-image-a}}
%\subfloat[Monodepth2]{
%\includegraphics[width=0.23\textwidth]{example-image-a}}
%\subfloat[Ours]{
%\includegraphics[width=0.23\textwidth]{example-image-a}}
%\setcounter{subfigure}{0}
\caption{Depth results on KITTI.}
\label{fig:kitti}
\end{figure*}

==> figures/other_uda.tex <==

\begin{figure*}[t!]
\centering
\subfloat[\emph{Parallel Domain} $\rightarrow$ \emph{Cityscapes}]{
\includegraphics[width=0.32\textwidth,height=3.8cm,trim=25 0 0 0,clip]{images/pd_ddad.png}}
\subfloat[\emph{VKITTI2} $\rightarrow$ \emph{KITTI}]{
\includegraphics[width=0.32\textwidth,height=3.8cm,trim=15 0 0 0,clip]{images/vkitti2_kitti.png}}
\subfloat[\emph{Parallel Domain} $\rightarrow$ \emph{DDAD}]{
\includegraphics[width=0.32\textwidth,height=3.8cm,trim=25 0 0 0,clip]{images/pd_ddad.png}}
\caption{\textbf{Semantic segmentation results on different UDA scenarios}, using GUDA.}
\label{fig:pd_ddad}
\end{figure*}




==> figures/scale_pd.tex <==

\begin{figure}[t!]
\centering
\includegraphics[width=0.48\textwidth]{images/scale_pd.png}
\caption{\textbf{Unsupervised domain adaptation results for semantic segmentation on \textit{Cityscapes}}, using different virtual datasets.}
\label{fig:scale_pd}
\vspace{-8mm}
\end{figure}

==> figures/synthia.tex <==

\begin{figure*}[t!]
\centering
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/pd/pd-01-rgb.png}} 
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/pd/pd-01-depth.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/pd/pd-01-pred_depth.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/pd/pd-01-normals.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/pd/pd-01-pred_normals.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/pd/pd-01-semantic.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/pd/pd-01-pred_semantic.png}}
\\
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-01-rgb.png}} 
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-01-depth.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-01-pred_depth.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-01-normals.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-01-pred_normals.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-01-semantic.png}}
\hspace{0.02mm}
\subfloat{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-01-pred_semantic.png}}
\\ \vspace{-3mm}
\setcounter{subfigure}{0}
\subfloat[Input RGB]{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-02-rgb.png}}
\hspace{0.02mm}
\subfloat[GT Depth]{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-02-depth.png}}
\hspace{0.02mm}
\subfloat[Pred. Depth]{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-02-pred_depth.png}}
\hspace{0.02mm}
\subfloat[GT Normals]{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-02-normals.png}}
\hspace{0.02mm}
\subfloat[Pred. Normals]{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-02-pred_normals.png}}
\hspace{0.02mm}
\subfloat[GT Semantic]{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-02-semantic.png}}
\hspace{0.02mm}
\subfloat[Pred. Semantic]{\includegraphics[width=0.12\textwidth,height=1.2cm]{images/synthia/synthia-02-pred_semantic.png}}
\caption{Results on different datasets.}
\label{fig:kitti}
\end{figure*}

==> figures/training.tex <==

\begin{figure*}[t!]
\centering
\subfloat{
\includegraphics[width=0.8\textwidth]{example-image-a}}
\caption{Predicted tasks on DDAD.}
\label{fig:training}
\end{figure*}

==> suppmat/dada.tex <==




\begin{table*}[t!]
\renewcommand{\arraystretch}{1.0}
\centering
{
\small
\setlength{\tabcolsep}{0.35em}
\begin{tabular}{l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c||c|c|}
\toprule
\multirow{3}{*}{\textbf{Method}}
& \multirow{3}{*}{\rotatebox{90}{Road}}
& \multirow{3}{*}{\rotatebox{90}{S.walk}}
& \multirow{3}{*}{\rotatebox{90}{Build.}} 
& \multirow{3}{*}{\rotatebox{90}{Wall*}}
& \multirow{3}{*}{\rotatebox{90}{Fence*}}
& \multirow{3}{*}{\rotatebox{90}{Pole*}}
& \multirow{3}{*}{\rotatebox{90}{T.Light}}
& \multirow{3}{*}{\rotatebox{90}{T.Sign}}
& \multirow{3}{*}{\rotatebox{90}{Vegt.}}
& \multirow{3}{*}{\rotatebox{90}{Sky}}
& \multirow{3}{*}{\rotatebox{90}{Person}}
& \multirow{3}{*}{\rotatebox{90}{Rider}}
& \multirow{3}{*}{\rotatebox{90}{Car}}
& \multirow{3}{*}{\rotatebox{90}{Bus}}
& \multirow{3}{*}{\rotatebox{90}{Motor.}}
& \multirow{3}{*}{\rotatebox{90}{Bike}}
& \multirow{3}{*}{\rotatebox{90}{mIoU}}
& \multirow{3}{*}{\rotatebox{90}{mIoU*}}
\\
& & & & & & & & & & & & & & & & & &
\\
& & & & & & & & & & & & & & & & & &
\\


\toprule
\multicolumn{19}{l}{\textbf{(a) SYNTHIA $\rightarrow$ Cityscapes}} \\
\toprule

DADA \cite{vu2019dada}
& 89.2 & 44.8 & 81.4 & 6.8 & 0.3 & 26.2 & 8.6 & 11.1 & 81.8 & 84.0 & 54.7 & 19.3 & 79.7 & 40.7 & 14.0 & 38.8 & 42.6 & 49.8 \\
DADA \cite{vu2019dada} $\dagger$
& 87.7 & 43.7 & 80.4 & 9.6 & 0.4 & 28.8 & 10.8 & 15.0 & 80.8 & 82.63 & 53.8 & 17.6 & 78.0 & 34.8 & 16.6 & 33.6 & 42.1 & - \\
\textbf{GUDA} 
& - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\

\cmidrule{1-19}
\multicolumn{19}{l}{\textbf{(c) SYNTHIA $\rightarrow$ 2 $\times$ Cityscapes}} \\
\cmidrule{1-19}

\textbf{DADA \cite{vu2019dada} $\dagger$} 
& - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 42.5 & - \\
\textbf{GUDA} 
& - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\

\cmidrule{1-19}
\multicolumn{19}{l}{\textbf{(c) SYNTHIA $\rightarrow$ 30 $\times$ Cityscapes}} \\
\cmidrule{1-19}
\textbf{DADA \cite{vu2019dada} $\dagger$} 
& - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
\textbf{GUDA} 
& 85.4 & 49.5 & 80.8 & 13.8 & 0.9 & 36.2 & 21.8 & 35.2 & 78.8 & 84.7 & 59.9 & 13.5 & 84.0 & 33.8 & 2.8 & 30.9 & 44.5 & 50.9 \\

\cmidrule{1-19}

\bottomrule

\end{tabular}
}
\caption{\textbf{Semantic segmentation results on \emph{Cityscapes}.} The \emph{mIoU} metric considers all 16 classes, and \emph{mIoU*} considers only the 13 classes present in SYNTHIA (removing the ones marked with \emph{*}). $\dagger$ denotes numbers replicated by us using publicly released code.} 
\label{tab:synthia_cs}
\vspace{-3mm}
\end{table*}

==> tables/old/cityscapes_depth.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& Virtual &
Abs.Rel &
Sqr.Rel &
RMSE &
RMSE$_{log}$ &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\toprule

%\parbox[t]{2mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{\textit{Eigen}}}}

Monodepth2
& VK2 & 0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981
\\
\textbf{Ours}
& VK2 & 0.108 & 0.762 & 4.606 & 0.191 & 0.879 & 0.961 & 0.982
\\
\bottomrule
\end{tabular}
}
\caption{Depth results on KITTI.} 
\label{tab:baseline}
\end{table*}

==> tables/old/datasets.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cc}

\toprule
& Depth & Semantic 
\\
\toprule

KITTI
& \checkmark & \checkmark 
\\
DDAD
& \checkmark & \checkmark 
\\
Cityscapes
& \checkmark & \checkmark 
\\
\midrule
\midrule
VKITTI2
& \checkmark & \checkmark
\\
CARLA
& $\circ$ & $\circ$
\\
PD
& \checkmark & \checkmark 
\\

\bottomrule

\end{tabular}
}
\caption{Datasets considered in this paper.} 
\label{tab:baseline}
\end{table*}



% \begin{table*}[t!]
% \renewcommand{\arraystretch}{1.00}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{l|ccc}

% \toprule
% & VKITTI2 & CARLA & Parallel Domain
% \\
% \toprule

% KITTI
% & --- & --- & --- 
% \\
% DDAD
% & --- & --- & --- 
% \\
% Cityscapes
% & --- & --- & --- 
% \\

% \bottomrule

% \end{tabular}
% }
% \caption{Datasets considered in this paper.} 
% \label{tab:baseline}
% \end{table*}






==> tables/old/ddad_depth.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|cccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
\multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& 
Abs.Rel &
Sqr.Rel &
RMSE &
RMSE$_{log}$ &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\toprule

Real
& 0.203 & 6.999 & 16.844 & 0.290 & 0.748 & 0.902 & 0.954
\\
Virtual
& 0.233 & 4.429 & 18.498 & 0.341 & 0.620 & 0.853 & 0.932
\\
Real (PT virtual)
& 0.173 & 3.846 & 19.025 & 0.301 & 0.737 & 0.887 & 0.943
\\
Virtual+Real
& 0.147 & 2.922 & 14.452 & 0.242 & 0.809 & 0.932 & 0.970
\\
\bottomrule
\end{tabular}
}
\caption{Depth results on DDAD.} 
\label{tab:baseline}
\end{table*}






==> tables/old/depth.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|l|c|cccc|ccc}
\toprule
& \multirow{2}{*}{\textbf{Method}} &
Sim. & \multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& & Dataset &
Abs.Rel &
Sqr.Rel &
RMSE &
RMSE$_{log}$ &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\toprule

\parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{KITTI}}}}

& Monodepth2 & --- & 
0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981
\\
& PackNet & --- & 
0.111 & 0.785 & 4.601 & 0.189 & 0.878 & 0.960 & 0.982
\\
& Ours & VK2 & 
0.108 & 0.762 & 4.606 & 0.191 & 0.879 & 0.961 & 0.982
\\

\midrule
\midrule

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{DDAD}}}}

& Ours (V) & PD &
0.233 & 4.429 & 18.498 & 0.341 & 0.620 & 0.853 & 0.932
\\
& Ours (R) & --- &
0.203 & 6.999 & 16.844 & 0.290 & 0.748 & 0.902 & 0.954
\\
& Ours (V $\rightarrow$ R) & PD &
0.173 & 3.846 & 19.025 & 0.301 & 0.737 & 0.887 & 0.943
\\
& Ours (V \leftrightarrow R) & PD &
0.147 & 2.922 & 14.452 & 0.242 & 0.809 & 0.932 & 0.970
\\

\midrule
\midrule

\parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textit{Cityscapes}}}}

& --- & --- &
--- & --- & --- & --- & --- & --- & ---
\\
& --- & --- &
--- & --- & --- & --- & --- & --- & ---
\\
& --- & --- &
--- & --- & --- & --- & --- & --- & ---
\\
& --- & --- &
--- & --- & --- & --- & --- & --- & ---
\\
& --- & --- &
--- & --- & --- & --- & --- & --- & ---
\\

\bottomrule

\end{tabular}
}
\caption{Depth results on different datasets.} 
\label{tab:depth}
\end{table*}

==> tables/old/kitti_depth.tex <==

\begin{table*}[t!]
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{l|c|cccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Method}} &
Sim. & \multicolumn{4}{|c|}{Lower is better $\downarrow$} &
\multicolumn{3}{|c}{Higher is better $\uparrow$} \\
& Dataset &
Abs.Rel &
Sqr.Rel &
RMSE &
RMSE$_{log}$ &
$\delta<1.25$ &
$\delta<1.25^2$ &
$\delta<1.25^3$\vspace{0.5mm}\\
\toprule

Monodepth2
& VK2 & 0.115 & 0.903 & 4.863 & 0.193 & 0.877 & 0.959 & 0.981
\\
\textbf{Ours}
& VK2 & 0.108 & 0.762 & 4.606 & 0.191 & 0.879 & 0.961 & 0.982
\\
\bottomrule
\end{tabular}
}
\caption{Depth results on KITTI.} 
\label{tab:baseline}
\end{table*}

==> tables/old/semantic.tex <==


\begin{table*}[t!]
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|c|c||l|r|l|l|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\toprule
& & & 
\multirow{4}{*}{\rotatebox{90}{Road}} &
\multirow{4}{*}{\rotatebox{90}{Sidewalk}} &
\multirow{4}{*}{\rotatebox{90}{Building}} & 
\multirow{4}{*}{\rotatebox{90}{Wall}} &
\multirow{4}{*}{\rotatebox{90}{Fence}} &
\multirow{4}{*}{\rotatebox{90}{Pole}} &
\multirow{4}{*}{\rotatebox{90}{T-Light}} &
\multirow{4}{*}{\rotatebox{90}{T-Sign}} &
\multirow{4}{*}{\rotatebox{90}{Vegetation}} &
\multirow{4}{*}{\rotatebox{90}{Sky}} &
\multirow{4}{*}{\rotatebox{90}{Person}} &
\multirow{4}{*}{\rotatebox{90}{Rider}} &
\multirow{4}{*}{\rotatebox{90}{Car}} &
\multirow{4}{*}{\rotatebox{90}{Bus}} &
\multirow{4}{*}{\rotatebox{90}{Motorcycle}} &
\multirow{4}{*}{\rotatebox{90}{Bycicle}} &
\multirow{4}{*}{\rotatebox{90}{Mean IoU}}
\\
& & & & & & & & & & & & & & & & & & & 
\\
&  & \textbf{Sim.} & & & & & & & & & & & & & & & & & 
\\
& \textbf{Method} & \textbf{Dataset} & & & & & & & & & & & & & & & & & \\

\toprule

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{KITTI}}}}

& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\

\midrule
\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{DDAD}}}}

& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\

\midrule

\parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{Cityscapes}}}}

& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- \\

\bottomrule

\end{tabular}
}
\caption{Semantic results on different datasets.} 
\label{tab:semantic}
\end{table*}


% \begin{table*}[t!]
% \renewcommand{\arraystretch}{1.00}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.3em}
% \begin{tabular}{c|l|c|cccccc}
% \toprule
% & \multirow{2}{*}{\textbf{Method}} &
% Sim. & & & & & & \\
% & & Dataset &
% Car &
% Person &
% Building & 
% Pole &
% Road &
% Vegetation &

% \toprule

% \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textit{KITTI}}}}

% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\
% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\
% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\

% \midrule
% \midrule

% \parbox[t]{2mm}{\multirow{4}{*}{\rotatebox[origin=c]{90}{\textit{DDAD}}}}

% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\
% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\
% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\
% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\

% \midrule
% \midrule

% \parbox[t]{2mm}{\multirow{5}{*}{\rotatebox[origin=c]{90}{\textit{Cityscapes}}}}

% & Ours (V) & PD &
% 54.2 & 30.9 & 69.2 & 27.7 & 83.8 & 71.9
% \\
% & Ours (V \leftrightarrow R) & PD &
% 64.7 & 33.4 & 71.0 & 29.9 & 86.2 & 74.4
% \\
% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\
% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\
% & --- & --- &
% --- & --- & --- & --- & --- & ---
% \\

% \bottomrule

% \end{tabular}
% }
% \caption{Semantic results on different datasets.} 
% \label{tab:semantic}
% \end{table*}

==> tables/scaling_pd.tex <==


\begin{table*}[t!]
\renewcommand{\arraystretch}{1.00}
\centering
{
\small
\setlength{\tabcolsep}{0.3em}
\begin{tabular}{c|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c||c|c|}
\toprule
& \multirow{4}{*}{\textbf{Method}}
& \multirow{4}{*}{\rotatebox{90}{Road}}
& \multirow{4}{*}{\rotatebox{90}{Sidewalk}}
& \multirow{4}{*}{\rotatebox{90}{Building}} 
& \multirow{4}{*}{\rotatebox{90}{Wall}}
& \multirow{4}{*}{\rotatebox{90}{Fence}}
& \multirow{4}{*}{\rotatebox{90}{Pole}}
& \multirow{4}{*}{\rotatebox{90}{T-Light}}
& \multirow{4}{*}{\rotatebox{90}{T-Sign}}
& \multirow{4}{*}{\rotatebox{90}{Vegetation}}
& \multirow{4}{*}{\rotatebox{90}{Sky}}
& \multirow{4}{*}{\rotatebox{90}{Person}}
& \multirow{4}{*}{\rotatebox{90}{Rider}}
& \multirow{4}{*}{\rotatebox{90}{Car}}
& \multirow{4}{*}{\rotatebox{90}{Bus}}
& \multirow{4}{*}{\rotatebox{90}{Motorcycle}}
& \multirow{4}{*}{\rotatebox{90}{Bycicle}}
& \multirow{4}{*}{\rotatebox{90}{mIoU}}
& \multirow{4}{*}{\rotatebox{90}{mIoU*}}
\\
& & & & & & & & & & & & & & & & & & &
\\
& & & & & & & & & & & & & & & & & & &
\\
& & & & & & & & & & & & & & & & & & &
\\

\toprule

\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{$320 \times 640$}}}

& PD v1.0
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & 39.4 & --- \\
& PD v1.0    
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & 40.7 & --- \\
& PD v1.2
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & 40.3 & --- \\
& PD v1.4   
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & 41.5 & --- \\
& PD v1.6   
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & 41.0 & --- \\
& PD v1.8      
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & 41.7 & --- \\
& PD v2.0      
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & 42.5 & --- \\

\midrule 
\midrule

\parbox[t]{2mm}{\multirow{6}{*}{\rotatebox[origin=c]{90}{$512 \times 1024$}}}

& PD v1.0 
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & 40.7 & --- \\
& PD v1.2
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- & --- \\
& PD v1.4 
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- & --- \\
& PD v1.6 
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- & --- \\
& PD v1.8 
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- & --- \\
& PD v2.0 
& --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & --- & ---  & --- & --- & --- & --- & --- & --- \\

\bottomrule

\end{tabular}
}
\caption{\textbf{Semantic Segmentation results on \textit{Parallel Domain} $\rightarrow$ \textit{Cityscapes}}, with increasing amounts of virtual data. } 
\label{tab:scaling_pd}
\end{table*}




==> tables/semantic_kitti_ddad.tex <==


% \begin{table}[t!]
% \renewcommand{\arraystretch}{1.00}
% \centering
% {
% \small
% \setlength{\tabcolsep}{0.25em}
% \begin{tabular}{|l||c|c|c|c|c|c|c|c|c|c|c|c|c|c||c|}
% \toprule
% \multirow{4}{*}{\textbf{Method}}
% & \multirow{4}{*}{\rotatebox{90}{Road}}
% & \multirow{4}{*}{\rotatebox{90}{Sidewalk}}
% & \multirow{4}{*}{\rotatebox{90}{Building}} 
% & \multirow{4}{*}{\rotatebox{90}{Pole}}
% & \multirow{4}{*}{\rotatebox{90}{T-Light}}
% & \multirow{4}{*}{\rotatebox{90}{T-Sign}}
% & \multirow{4}{*}{\rotatebox{90}{Vegetation}}
% & \multirow{4}{*}{\rotatebox{90}{Terrain}}
% & \multirow{4}{*}{\rotatebox{90}{Sky}}
% & \multirow{4}{*}{\rotatebox{90}{Person}}
% & \multirow{4}{*}{\rotatebox{90}{Rider}}
% & \multirow{4}{*}{\rotatebox{90}{Car}}
% & \multirow{4}{*}{\rotatebox{90}{Bus}}
% & \multirow{4}{*}{\rotatebox{90}{Truck}}
% & \multirow{4}{*}{\rotatebox{90}{mIoU}}
% \\
% & & & & & & & & & & & & & & & 
% \\
% & & & & & & & & & & & & & & & 
% \\
% & & & & & & & & & & & & & & & 
% \\
% \midrule
% %\parbox[t]{2mm}{\multirow{17}{*}{\rotatebox[origin=c]{90}{}}}

% \textbf{GUDA} 
% & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 & 00.0 \\

% \cmidrule{1-16}

% \bottomrule

% \end{tabular}
% }
% \caption{\textbf{Semantic segmentation results on \textit{SYNTHIA} $\rightarrow$ \textit{Cityscapes}}, considering different unsupervised domain adaptation methods. The \emph{mIoU} metric considers all 16 classes, and \emph{mIoU*} considers only 13 classes.} 
% \label{tab:synthia_cs}
% \end{table}


